Goal Translation for a Hammer for Coq (Extended Abstract)

Hammers are tools that provide general purpose automation for formal proof assistants. Despite the gaining popularity of the more advanced versions of type theory, there are no hammers for such systems. We present an extension of the various hammer components to type theory: (i) a translation of a significant part of the Coq logic into the format of automated proof systems; (ii) a proof reconstruction mechanism based on a Ben-Yelles-type algorithm combined with limited rewriting, congruence closure and a first-order generalization of the left rules of Dyckhoff's system LJT.

==> eptcsdata.tex <==
\providecommand{\firstpage}{13}
\providecommand{\publicationstatus}{J.C. Blanchette and C. Kaliszyk:\\
Hammers for Type Theories (HaTT'16)\\
EPTCS 210, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.210.4}{10.4204/EPTCS.210.4}}

